Recovery from Link Failures in Networks with Arbitrary Topology via Diversity Coding

Link failures in wide area networks are common. To recover from such failures, a number of methods such as SONET rings, protection cycles, and source rerouting have been investigated. Two important considerations in such approaches are the recovery time and the needed spare capacity to complete the recovery. Usually, these techniques attempt to achieve a recovery time less than 50 ms. In this paper we introduce an approach that provides link failure recovery in a hitless manner, or without any appreciable delay. This is achieved by means of a method called diversity coding. We present an algorithm for the design of an overlay network to achieve recovery from single link failures in arbitrary networks via diversity coding. This algorithm is designed to minimize spare capacity for recovery. We compare the recovery time and spare capacity performance of this algorithm against conventional techniques in terms of recovery time, spare capacity, and a joint metric called Quality of Recovery (QoR). QoR incorporates both the spare capacity percentages and worst case recovery times. Based on these results, we conclude that the proposed technique provides much shorter recovery times while achieving similar extra capacity, or better QoR performance overall.

==> algorithm2e/algorithm2e/algorithm2e_ex01.tex <==
\SetAlgoVlined
\eIf{cond1}{
  a line\;
  a line\;
}{
  another line\;
  another line\;
}


==> algorithm2e/algorithm2e/algorithm2e_ex02.tex <==
\SetAlgoNoLine
\If{cond2}{
  second if\;
  second if\;
}


==> algorithm2e/algorithm2e/algorithm2e_ex03.tex <==
\lIf{cond3}{ another example}
\Else{
  a block\;
  a block\;
}


==> algorithm2e/algorithm2e/algorithm2e_ex04.tex <==
\lIf{cond4}{ok} \lElse{wrong}\;

==> algorithm2e/algorithm2e/algorithm2e_ex05.tex <==
\SetAlgoVlined
\lIf{cond5}{cond5 true}\;
\uElseIf{cond51}{
  cond 5 false\;
  but cond51 true\;
}
\ElseIf{}{
  all is wrong\;
  \Return result52\;
}


==> algorithm2e/algorithm2e/algorithm2e_ex06.tex <==
\SetAlgoLined
\uIf{cond6}{
  cond6 is ok\;
  always ok\;
}
\uElseIf{cond62}{
  choose result62\;
  \Return result62\;
}
\Else{
  all is wrong\;
  do something else\;
}


==> algorithm2e/algorithm2e/algorithm2e_ex07.tex <==
Let's have a look at what we can do
with if-then-else and side comments\;
\eIf{if-then-else test}{
  no comment here\;
  neither in then\;
}{
  nor in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  then with a comment\;
}(\tcc*[f]{comment in else})
{
  here we are in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  again a comment in then\;
}{
  but not in else\;
}
\eIf{if-then-else test}{
  this time, no comment in then\;
}(\tcc*[f]{else comment})
{
  but one comment in else\;
}
Let's try with other if possibilities\;
\lIf(\tcc*[h]{lif comment}){test}{text}
\uIf(\tcc*[f]{uif comment}){test}{
  then text\;
}
\uElseIf(\tcc*[f]{comment}){test}{
  elseif text\;
}
\lElseIf(\tcc*[h]{comment}){test}{text}
\lElse(\tcc*[f]{comment}){text}


==> algorithm2e/algorithm2e/algorithm2e_exAlgoDisjdecomp.tex <==
\IncMargin{1em}
\begin{algorithm}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

  \Input{A bitmap $Im$ of size $w\times l$}
  \Output{A partition of the bitmap}
  \BlankLine
  \emph{special treatment of the first line}\;
  \For{$i\leftarrow 2$ \KwTo $l$}{
    \emph{special treatment of the first element of line $i$}\;
    \For{$j\leftarrow 2$ \KwTo $w$}{\label{forins}
      \Left$\leftarrow$ \FindCompress{$Im[i,j-1]$}\;
      \Up$\leftarrow$ \FindCompress{$Im[i-1,]$}\;
      \This$\leftarrow$ \FindCompress{$Im[i,j]$}\;
      \If(\tcp*[h]{O(\Left,\This)==1}){\Left compatible with \This}{\label{lt}
        \lIf{\Left $<$ \This}{\Union{\Left,\This}}\;
        \lElse{\Union{\This,\Left}\;}
      }
      \If(\tcp*[f]{O(\Up,\This)==1}){\Up compatible with \This}{\label{ut}
        \lIf{\Up $<$ \This}{\Union{\Up,\This}}\;
        \tcp{\This is put under \Up to keep tree as flat as possible}\label{cmt}
        \lElse{\Union{\This,\Up}}\tcp*[r]{\This linked to \Up}\label{lelse}
      }
    }
    \lForEach{element $e$ of the line $i$}{\FindCompress{p}}
  }
  \caption{disjoint decomposition}\label{algo_disjdecomp}
\end{algorithm}\DecMargin{1em}

==> algorithm2e/algorithm2e/algorithm2e_exIR.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwData{$G=(X,U)$ such that $G^{tc}$ is an order.}
\KwResult{$G'=(X,V)$ with $V\subseteq U$ such that $G'^{tc}$ is an
interval order.}
\Begin{
  $V \longleftarrow U$\;
  $S \longleftarrow \emptyset$\; 
  \For{$x\in X$}{ 
    $NbSuccInS(x) \longleftarrow 0$\;
    $NbPredInMin(x) \longleftarrow 0$\;
    $NbPredNotInMin(x) \longleftarrow |ImPred(x)|$\;
    }
  \For{$x \in X$}{
    \If{$NbPredInMin(x) = 0$ {\bf and} $NbPredNotInMin(x) = 0$}{
      $AppendToMin(x)$}
    } 
    \nl\While{$S \neq \emptyset$}{\label{InRes1}
    \nlset{REM} remove $x$ from the list of $T$ of maximal index\;\label{InResR}
    \lnl{InRes2}\While{$|S \cap  ImSucc(x)| \neq |S|$}{ 
      \For{$ y \in  S-ImSucc(x)$}{
        \{ remove from $V$ all the arcs $zy$ : \}\;
        \For{$z \in  ImPred(y) \cap  Min$}{
          remove the arc $zy$ from $V$\;
          $NbSuccInS(z) \longleftarrow NbSuccInS(z) - 1$\;
          move $z$ in $T$ to the list preceding its present list\;
          \{i.e. If $z \in T[k]$, move $z$ from $T[k]$ to 
           $T[k-1]$\}\;
          }
        $NbPredInMin(y) \longleftarrow 0$\;
        $NbPredNotInMin(y) \longleftarrow 0$\;
        $S \longleftarrow S - \{y\}$\;
        $AppendToMin(y)$\;
        }
      }
    $RemoveFromMin(x)$\;
    }
  }  
\caption{IntervalRestriction\label{IR}}
\end{algorithm}


==> algorithm2e/algorithm2e/algorithm2e_exfor.tex <==
\SetAlgoLined
\ForAll{elements of $S_1$}{
  remove an element e from $S_1$\;
  put e in the set $S_2$\;
  }
\lFor{i=1 \emph{\KwTo}max}{mark i}\;
\ForEach{$e$ in the set}{
  put $e$ in ${\cal E}$\;
  mark $e$\;
}


==> algorithm2e/algorithm2e/algorithm2e_exrepeat.tex <==
\Repeat{this stop condition}{
  the text of the loop\;
  another line\;
  always in the loop\;
  }
\lRepeat{stop}{a one line loop}


==> algorithm2e/algorithm2e/algorithm2e_exswitch.tex <==
\Switch{the value of T}{
  \uCase{a value}{
    do this\;
    do that\;
  }
  \lCase{another value}{one line}\;
  \Case{last value}{
    do this\;
    break\;
  }
  \Other{
    for the other values\;
    do that\;
  }
}


==> comparisons.tex <==
\section{Technical Comparisons of Different Techniques}
   This section is devoted to compare technical properties of diversity coding with previously mentioned protection techniques, which are shared backup path protection and p-cycles.  Evaluating the performance of different protection techniques can be investigated many subsections; such as spare capacity percentage, recovery duration, design complexity, hardware complexity. In this section, the most concerned properties of protection schemes are discussed and compared. The list of most important feature of protection scheme consist of \cite{vasseur}.

\begin{itemize}
\item Scope of failure coverage
\item  Spare capacity percentage
\item Recovery duration
\item Hardware complexity
\item Design complexity
\item Scalability
\end{itemize}

   We reserve the discussion about spare capacity percentage to next section, which will be given in more detail and follow the list with recovery duration. Diversity coding offers full coverage from any single link failure. Proper adjustments are made so that p-cycles and sbpp have full coverage from any single link failure.

   Even there are opposition \cite{GroverBook}, there is a strong motivation behind developing faster protection schemes which goes under 50 ms recovery duration. The mesh-type protection schemes are known as slow techniques, which is also same case for shared backup path protection, however p-cycles are claimed to satisfy this 50 ms limit for recovery from any single link failure. At p-cycles, only end nodes of a failure have a workload of detecting the failure and rerouting the traffic bandwidth through multiple p-cycles. The cross-connections at p-cycles are pre-configured which speeds up the recovery from the failure. At sbpp, end nodes of a demand are noticed after a failure occurrence and all nodes, either on working path or spare path, take action and bandwidth assignments are transferred from working paths to spare paths. On the other hand, diversity coding is even faster than p-cycles method. Because only factor, that adds up recovery duration, is time shift of the duplicated signal that traverses over spare path. This shift consists of and duration of an XOR operation and propagation delay of signal between receiver node and decoding node.
As it is mentioned sbpp and p-cycles employ control mechanisms and require dynamic cross-connections depending on the network state. Therefore, the hardware complexity of these two techniques is higher than diversity coding, which has no dynamic post-configuration workload.

   Diversity coding is more scalable technique than p-cycles and sbpp. When the network size and traffic bandwidth increase , complexity of sbpp exponentially increases, since the number of nodes and connections involved in single link failure scenario exponentially increases. P-cycles suffer from spare capacity percentage as network size gets bigger because there is a limit of maximum cycle size and p-cycle technique gets far away from being optimal. In addition, increasing traffic bandwidth force p-cycle algorithm to employ a larger number different cycles per end-to end demand, which adds to complexity p-cycles. On the other hand, larger network size is advantageous for diversity coding, since spare capacity percentage is inversely related to average hop distance of an end-to end demand. Larger network size adds to design complexity diversity coding, as well as p-cycles and sbpp. It can be concluded that diversity coding is a better technique in terms of scalability.

